Knowledge-Aware Graph-Enhanced GPT-2 for Dialogue State Tracking

Dialogue State Tracking is central to multi-domain task-oriented dialogue systems, responsible for extracting information from user utterances. We present a novel hybrid architecture that augments GPT-2 with representations derived from Graph Attention Networks in such a way to allow causal, sequential prediction of slot values. The model architecture captures inter-slot relationships and dependencies across domains that otherwise can be lost in sequential prediction. We report improvements in state tracking performance in MultiWOZ 2.0 against a strong GPT-2 baseline and investigate a simplified sparse training scenario in which DST models are trained only on session-level annotations but evaluated at the turn level. We further report detailed analyses to demonstrate the effectiveness of graph models in DST by showing that the proposed graph modules capture inter-slot dependencies and improve the predictions of values that are common to multiple domains.

==> pages/Introduction_backup.tex <==
\section{Introduction}
\label{sec:introduction}

% Building dialogue systems that can converse with users engagingly and coherently is a long-standing goal of developing Artificial intelligence (AI).
% In recent years, dialogue systems have seized great attention from academia and industry due to the rapid development of machine-learning-based approaches and the increasing amount of data available to train these models \cite{chen2017survey}. Multi-domain task-oriented dialogue systems are a promising research direction that are designed to address multiple pre-defined tasks of several domains including booking of restaurants, hotels, trains, and taxis, and seeking help from the police and hospitals. 
%There are mainly two types of dialogue bots under active investigations: open-domain and multi-domain. Open-domain dialogue systems aim to establish long-term connections with users by satisfying their needs for communication, affection, social belonging, and information retrieval \cite{chen2017survey}.
%They are built for solving the requests from users efficiently and exactly.
% These tasks include booking of restaurants, hotels, trains, and taxis, and seeking help from the police and hospitals.

% Multi-domain task-oriented dialogue systems are designed to address multiple pre-defined tasks of several domains including booking of restaurants, hotels, trains, and taxis, and seeking help from the police and hospitals. 
A key component of multi-domain systems is the dialogue state tracker (DST) which extracts values of domain-slot pairs (e.g. \texttt{<hotel-pricerange>} is a domain-slot pair associated with hotel price range) from the dialogue history and determine slot values (e.g. expensive/moderate/cheap) for later system actions such as booking.
Even though DSTs are mature, the performance of such trackers still limits overall system performance.
% Most of the recent machine-learning models only achieved around 53\% in joint accuracy in a commonly-used benchmark dataset - MultiWOZ 2.0 \cite{budzianowski2018multiwoz}.
The difficulty of achieving better results comes mainly from the complexity of the tasks they address.
For instance, there are 30 different domain-slot pairs in MultiWOZ 2.0 \cite{budzianowski2018multiwoz}, each being a task where a system needs to classify among hundreds of possible candidates.

\textbf{Sparsely supervised} DST learning has recently seized the attention of researchers \cite{liang2021attention}.
Unlike turn-level annotations for which annotators label all intermediate turn states through the whole dialogue session, session-level annotations are significantly easier to be obtained.
For example, after customer phone calls, session-level annotations can be obtained easily from telephone operators by the recorded system actions \cite{liang2021attention} or the information that has been noted down.
% In practical scenarios, it is always easier for telephone operators to collect state labels for the entire session after phone calls rather than annotating all the intermediate states when a session is ongoing.
% Such session-level last-turn annotations can also be quickly collected by the operator actions (e.g. APIs) \cite{liang2021attention}.
Therefore, if the DST learning is limited to use only those session-level labels but still achieves an acceptable performance,
the acquisition of new DST datasets will be benefited by easier collection and fewer required samples.
For example, the session-level samples of last turns of dialogues in MultiWOZ 2.0
% ~\cite{eric2019multiwoz}
only take up around 14.3\% of the original samples.
% Therefore, if the DST learning can utilize only last-turn labels, which leads to a \textbf{sparse supervision} scheme, the samples required to build a dataset will be significantly reduced by around 10 times. For example, the last-turn samples in MultiWOZ 2.0~\cite{eric2019multiwoz} only take up around 14.3\% of the original samples.
% As introduced in Sec.\ref{sec:introduction}, it is beneficial to the industry and larger volume of multi-domain data may become feasible if our models can retain performance with sparse supervision (trained with last-turn samples only).
% The training samples are reduced from $54 ,971$ to only $7,884$ ($14.3\%$), 
% and thus we expect a performance drop due to the hugely reduced number of training samples.

Recently, the idea of utilizing the relationship between domain-slots was explored by \citeauthor{zhou2019multi} \citeyearpar{zhou2019multi}
and they explained three types of relationships that are useful:
% There are three types of relationships that are useful:
(1) Two domain-slot pairs with the same candidate set, e.g. \texttt{<restaurant-bookday>} has the same possible candidate set as \texttt{<hotel-bookday>};
(2) The candidate set of a domain-slot is a subset of that of another domain-slot, e.g. the candidate set of \texttt{<restaurant-name>} is a subset of that of \texttt{<taxi-destination>};
(3) two domain-slot pairs have correlated values, e.g. the star level of the booked hotel correlates with the price range of the reserved restaurant.

The aforementioned relationships may bridge slots by utilizing value dependencies
especially when 
the number of domain-slots being evaluated increases or when available samples reduces dramatically in sparse supervision training.
Such relationships can be represented by edges in knowledge graphs, where domains, slots, and values are graph nodes.
Therefore, Graph Neural Networks (GNNs) were proposed to exploit the interactions among slots and values and improved the DST performance substantially \cite{zhou2019multi, 0002LWZT020}.
% Therefore, Graph Neural Networks (GNNs) have exhibited great potentials in improving the performance of DST 
% by utilizing the interaction between slots and values \cite{zhou2019multi, 0002LWZT020}, and it is a straight intuition to utilize GNNs in facilitating model learning when slots are bridged by some relationships.
% training samples are from the last turns only, because GNNs may be able to capture the inter-slot relations in the last turn, and help model retain performance at the intermediate turns.
However, none of the work cited above has explored quantitatively and explained in depth how graph models utilize the relationships they mentioned.
For example, \citeauthor{0002LWZT020} ~\citeyearpar{0002LWZT020} provided one single example where the predictions of correlated values were potentially enhanced by their model, while \citeauthor{zhou2019multi}~\citeyearpar{zhou2019multi} only presented an ablation study formed by their models with/without graphs.
Therefore, this paper will try to answer this question with more details and demonstrate how graph models benefit the learning of models.
% , which, in our opinion, is important to support the effectiveness of graph models.


Furthermore, graph models may help to compensate for the drawbacks of generative models.
Each dialogue state value may consists of more than one token, and as a result, recent models using bi-directional attention mechanisms (such as BERT \cite{devlin-etal-2019-bert}) usually have to utilize span predictions or embedding-based classifications (e.g. \citeauthor{shan-etal-2020-contextual}~\citeyearpar{shan-etal-2020-contextual}) due to the fact that in practice they do not handle the generation of possibly very long value outputs well.
As a well-known generative model, GPT-2~\cite{radford2019language} features its power of causal left-to-right generation with single-direction attentions, and \citet{NEURIPS2020_e9462095} showed that it can extract slot values of variable lengths token by token sequentially with the aid of some special tokens separating slots.
However, the single-direction attention introduces causality that the prediction of later slot values take the information from the previously predicted slots explicitly, but not in the other direction, leading to a decreased performance for slots placed in front.
Therefore, we present a novel integration of GPT-2 and GATs, where GATs enable information exchange between slots to exploit value dependencies, while front slots can also communicate with later slots to mitigate the effect of causality.
% However, our design enables such causality to be compensated by allowing pre-extracted domain-slot features to exchange information before being used in predictions, which utilizes the generation power of GPT-2 while keeping all slots communicate effectively.

We summarize the contributions of our work as follows:

% (1) We propose a novel graph-enhanced GPT-2\cite{radford2019language}-based model which utilizes Graph Attention Networks (GATs) to allow inter-slot information exchange and perform slot-filling with a causal generation setting rather than the popular classification-based setting.
(1) We propose a novel architecture integration of GPT-2 with Graph Attention Networks (GATs) for the task of dialogue state tracking.
The model is shown to be robust when training samples are significantly reduced under sparse supervision.

(2) We demonstrate that our architecture also mitigates the issue that DSTs based on GPT-2 alone have, given that domain-slots are generated in a Left-to-Right manner.

(3) We elucidate how our knowledge-aware model exploits the relationships between domain-slots, and further demonstrate how the graph modules improves the predictions of dependent slot values.

%which have not been well analysed and explained in the literature.

%We perform three independent set of analysis to elucidate why such a model architecture is beneficial for Dialogue State Tracking. W

% (3) We show that our model is robust to hugely reduced number of samples, which 

% We further demonstrate how a graph  module retains performance when the model is sparsely supervised with only last-turn samples of dialogue sessions.

% (3) We conduct detailed error analyses to demonstrate what inter-slot correlations are concerned and how graph models improve the system performance by utilizing these relations, which have not been well analysed in the literature.
% (3) By detailed analyses, we elucidate how our grptaph module exploits the relationships between different domain-slots, which have not been well analysed and explained in the literature.

==> pages/Related_work_backup.tex <==
\section{Related Work}
% Traditional dialogue state tracking utilize language understanding modules to extract the semantics and then infer dialogue states, but they rely on handcrafted features.
\textbf{Dialogue State Trackers} traditioinally relies heavily on pre-defined domain-specific lexicons and handcrafted rules/features for extracting semantics and then determining the most probable slot values \citep{WILLIAMS2007393, THOMSON2010562, williams-2014-web}.
As a result, these systems face difficulty in scaling into new domains.



Most recent work in DST prioritize the need of building more general and extensible systems, and machine-learning architectures gained popularity in an extensive amount of publications \cite{wu-etal-2019-transferable, zhang2019find, huang-etal-2020-meta, lee2020sumbt+}.
% There have been an extensive amount of publications investigating machine-learning-based DST models~\cite{wu-etal-2020-tod, wu-etal-2019-transferable, zhang2019find, huang-etal-2020-meta, lee2020sumbt+}.
Most of these recent models utilize discriminative models, which are either trained to classify among all possible candidates, or predict start/end span indices to locate the occurrences of correct dialogue state values in the sentences.
Enumerable slots (with limited number of value candidates) are easier to be handled by the former approach while the latter finds non-enumerable slots (e.g. time-related slots with unlimited number of possible values) more efficiently.
Therefore, the recent trend is to combine multiple strategies to deal with the two types of values differently.
% , given that pure classification may be overwhelmed by huge candidate sets.
For example, \citet{zhang2019find} combines a span predictor for non-enumerable slot values and a cosine similarity matching that exploits a BERT model to extract representations for enumerable slot values, with which the dual-strategy model jointly handles both types of slot values.
\citet{zhou2019multi} runs a span predictor and a candidate classifier, and combines the decisions with gating functions.
Similarly, \citet{heck-etal-2020-trippy} selects slot values from separate components and aggregates to a final decision.

Generative models (e.g. GPT-2) are less popular in DST tasks, as they raise additional challenges for information aggregation subject to the causality, as discussed in Sec.~\ref{sec:introduction} . But they were recently shown to be competitive by \citet{NEURIPS2020_e9462095}.

\textbf{Few-shot DST Learning} is motivated by the reduced need for training samples and quicker adaption to new domains when models are pre-trained on large unspecialized corpora.
\citet{wu-etal-2019-transferable} proposed a transferable dialogue state generator that trains a copy mechanism and facilitates knowledge transfer when predicting unseen domain-slots.
\citet{wu-etal-2020-tod} tested a BERT-based model with weak supervision settings and a sharp performance decrease was observed.
The concept of sparse supervision in this paper was firstly proposed and experimented by \citet{liang2021attention}, but the performance of such scheme is still not satisfying.
% We present only work that are most relevant.
% For example, \citet{wu-etal-2019-transferable} proposed a transferable dialogue state generator that predicts dialogue states using a copy mechanism and facilitates knowledge transfer when predicting unseen domain-slots.
% \citet{zhang2019find} utilized two BERT models: one is to perform span predictions and the other one carries out
% Sparse supervision with last-turn samples was firstly proposed and experimented by \citet{liang2021attention}, but the performance of such scheme is still not satisfying.

\textbf{Sharing Information among Slots} either by explicitly copying \cite{ouyang-etal-2020-dialogue} or by embedding sharing \cite{hu-etal-2020-sas, zhou2019multi, 0002LWZT020} has been actively explored recently.
For example, TripPy framework \citep{heck-etal-2020-trippy} adopts explicit copying of values of other slots to exploit the value coreferences.
Graphs showed increasing potentials in implicit information sharing among slots, for example,
\citet{zhou2019multi} incorporated a graph attention network to further improve model performance, while a schema-guided multi-domain DST \cite{0002LWZT020} was proposed to embed slot relations in graph edges.
But these two work did not investigate in depth the interactions happening in knowledge graphs and did not provide insights into using graphs efficiently.
% and investigated the effects of different graph topology and graph hyperparameters (e.g. number of graph layers).



==> pages/Task_formulation.tex <==
\subsection{Task Formulation}
\label{sec:task_formulation}
% The state extraction can be formuated as a Q\&A task, as proposed by \citeauthor{zhou2019multi}~ \citeyearpar{zhou2019multi}.
There are $N_d$ domains and $N_{ds}$ domain-slot pairs.
There are $N_v$ value candidates that can appear as slot values given by the dataset.
% The dialogue state extraction is formulated as asking a question $Q_{ds_i}$ about the specific domain-slot pair $ds_i$.
The DST is required to fill the correct values to each of the $N_{ds}$ slots. For example, it can fill high, moderate, or cheap to \texttt{hotel-pricerange}, and fill 17:45 to \texttt{taxi-arriveBy}.


% answer either a value in the available value set of $d-s$ (e.g., high, moderate, or cheap in \texttt{hotel-pricerange}) or a non-enumerable answer from the user utterance (e.g., 17:45 for \texttt{taxi-arriveBy}).
% For generative models (e.g. GPT2), the model is required to generate the correct value directly.


